Query-Focused Opinion Summarization for User-Generated Content

We present a submodular function-based framework for query-focused opinion summarization. Within our framework, relevance ordering produced by a statistical ranker, and information coverage with respect to topic distribution and diverse viewpoints are both encoded as submodular functions. Dispersion functions are utilized to minimize the redundancy. We are the first to evaluate different metrics of text similarity for submodularity-based summarization methods. By experimenting on community QA and blog summarization, we show that our system outperforms state-of-the-art approaches in both automatic evaluation and human evaluation. A human evaluation task is conducted on Amazon Mechanical Turk with scale, and shows that our systems are able to generate summaries of high overall quality and information diversity.

==> framework.tex <==


%Our query-focused opinion summarization framework consists of three main components: \textit{Opinion Question Classification}, \textit{Candidate Ranking}, and \textit{Submodular Opinion Summarization}. In this section, we introduce the first two components, leaving our main method description in Section~\ref{sec:submodular}.

%\subsection{Opinion Question Classification}
%\label{subsec:opinQuestion}
%Our opinion question identification classifier is trained on two opinion question datasets on community QA that are from~\newcite{DBLP:conf/emnlp/LiLA08} and~\newcite{conf/aaai/AmiriZC13}. \newcite{DBLP:conf/emnlp/LiLA08} contains explicit opinion questions which usually contain strong sentiment words. A sample question is ``What is the ideal honeymoon destination which combines beach and adventure?". \newcite{conf/aaai/AmiriZC13} collect implicit opinion questions, such as ``what can you do to help environment?". We use them both to have a higher recall on the opinion questions.
%
%Since the questions in blog summarization data used in this work are all opinionated, this step is only carried out for community QA summarization. We utilize RBF-kernel based Support Vector Machines~\cite{Joachims:1999:MLS:299094.299104} implemented by LIBSVM~\cite{libsvm} as the classifier. Features are mostly adopted from existing work~\cite{DBLP:conf/emnlp/LiLA08,conf/aaai/AmiriZC13}, including \texttt{unigrams/bigrams}, \texttt{initial unigram/bigram/trigram}, \texttt{number of sentiment words}, \texttt{number of answers}, \texttt{average number of sentiment words in answers}.

%\subsection{Candidate Ranking}
%Statistical ranker has been widely used for opinion retrieval~\cite{DBLP:conf/cikm/ZhangYM07,Aktolga:2013:SDD:2484028.2484060}, and also proposed for answering opinion questions~\cite{conf/acl/LiTHZ09}. We also utilize statistical rankers to produce a preference ordering of the candidate answers or sentences. 
%The output of our ranker is transformed into a submodular function, and encoded as part of our final objective function for summarization along with other components that are capable to encourage diversity of the summary.
%
%ListNet~\cite{Cao:2007:LRP:1273496.1273513}, which has been shown effective in many information retrieval tasks, is chosen as our ranker. We use the implementation from Ranklib~\cite{citeulike:9435511}.
%
%Features used in the ranking algorithm are summarized in Table~\ref{tab:feature_ranking}. All features are normalized by standardization. Due to the length limit, we choose to describe key features only.
%[ATTN:Hema, could you please add description for MMP]
%
%\begin{table}
%    {\small
%    \setlength{\baselineskip}{0pt}
%    \begin{tabular}{|l|}
%    \hline
%    {\bf Basic Features}\\ \hline
%    answer position in all answers/sentence position in blog\\
%    length of the answer/sentence\\
%    length is less than 5 words\\
%    \hline
%    
%	{\bf Query-Independent Features}\\ \hline
%	unigram/bigram TFIDF similarity with cluster centroid\\
%	sumBasic score~\cite{nenkova-vanderwende-2005}\\
%	number of topic signature words~\cite{Lin:2000:AAT:990820.990892}\\
%    	JS divergence with cluster\\
%    \hline    
%    
%    {\bf Query-Relevant Features}\\ \hline
%    unigram/bigram TF/TFIDF similarity with query\\
%    	number of MMP~\cite{DBLP:conf/naacl/LuoRCMF13}\\
%    \hline
%    
%    {\bf Sentiment Features}\\ \hline    
%	number/portion of sentiment words\\
%	contains sentiment words with the same polarity as query\\
%
%    \hline    
%    
%    \end{tabular}
%    }
%    \vspace{-1mm}
%    \caption{\fontsize{10}{12}\selectfont Features used for candidate ranking. We use them both for ranking answers in community QA and }
%    \label{tab:feature_ranking}
%
%\end{table}





